EcoTTA: Memory-Efficient Continual Test-time Adaptation via Self-distilled Regularization

This paper presents a simple yet effective approach that improves continual test-time adaptation (TTA) in a memory-efficient manner. TTA may primarily be conducted on edge devices with limited memory, so reducing memory is crucial but has been overlooked in previous TTA studies. In addition, long-term adaptation often leads to catastrophic forgetting and error accumulation, which hinders applying TTA in real-world deployments. Our approach consists of two components to address these issues. First, we present lightweight meta networks that can adapt the frozen original networks to the target domain. This novel architecture minimizes memory consumption by decreasing the size of intermediate activations required for backpropagation. Second, our novel self-distilled regularization controls the output of the meta networks not to deviate significantly from the output of the frozen original networks, thereby preserving well-trained knowledge from the source domain. Without additional memory, this regularization prevents error accumulation and catastrophic forgetting, resulting in stable performance even in long-term test-time adaptation. We demonstrate that our simple yet effective strategy outperforms other state-of-the-art methods on various benchmarks for image classification and semantic segmentation tasks. Notably, our proposed method with ResNet-50 and WideResNet-40 takes 86% and 80% less memory than the recent state-of-the-art method, CoTTA.

==> table/supple_full_cifar10.tex <==
{\renewcommand{\arraystretch}{.95}
\begin{table*}
\centering
\arrayrulecolor{black}
\footnotesize
\vspace{-0.2cm}
\resizebox{.98\textwidth}{!}{
\begin{tabular}{l|l|ccccccccccccccc|c|c|}
\toprule
\textbf{Backbone}                                                              & \textbf{Method}         & Gaus. & Shot & Impu. & Defo. & Glas. & Moti. & Zoom & Snow & Fros. & Fog  & Brig. & Cont. & Elas. & Pixe. & Jpeg &  \textbf{Avg. err {\scriptsize $\downarrow$}} & \textbf{Mem. {\scriptsize $\downarrow$}}   \\
\drule
\multirow{11}{*}{\begin{tabular}[c]{@{}l@{}}WRN40 \\(Aug Mix)\end{tabular}} & Source         & 44.3  & 37.0 & 44.8  & 30.6  & 43.9  & 32.6  & 29.4 & 23.9 & 30.1  & 39.7 & 12.9  & 66.4  & 32.7  & 58.4  & 23.5 & 36.7  & 2                        \\
                                                                            & tBN            & 19.5  & 17.6 & 23.8  & 9.6   & 23.1  & 11.1  & 10.3 & 13.4 & 14.2  & 15.0 & 8.0   & 13.9  & 17.3  & 16.0  & 18.8 & 15.4  & 2                        \\
                                                                            & TENT online    & 16.4  & 13.9 & 19.1  & 8.3   & 19.1  & 9.3   & 8.6  & 10.9 & 11.3  & 12.0 & 6.9   & 11.6  & 14.6  & 12.2  & 15.6 & 12.7  & 188                      \\
                                                                            & TENT continual & 16.4  & 12.2 & 17.1  & 9.1   & 18.7  & 11.4  & 10.4 & 12.7 & 12.4  & 14.8 & 10.1  & 13.0  & 17.0  & 13.3  & 19.0 & 13.3  & 188                      \\
                                                                            & TTT++*         & 19.1  & 16.9 & 22.2  & 9.3   & 21.6  & 10.8  & 9.8  & 12.7 & 13.1  & 14.3 & 7.8   & 13.9  & 15.9  & 14.2  & 17.2 & 14.6  & 391                      \\
                                                                            & SWRNSP         & 15.9  & 13.3 & 18.2  & 8.4   & 18.5  & 9.5   & 8.6  & 11.0 & 10.2  & 11.7 & 7.0   & 8.1   & 14.6  & 11.3  & 15.1 & 12.1  & 400                     \\
                                                                            & NOTE           & 19.6  & 16.4 & 19.9  & 9.4   & 20.3  & 10.3  & 10.1 & 11.6 & 10.6  & 13.3 & 7.9   & 7.7   & 15.4  & 12.0  & 17.3 & 13.4  & 188                      \\
                                                                            & ETAT           & 15.2  & 13.1 & 17.5  & 9.5   & 19.9  & 11.6  & 9.3  & 11.4 & 11.5  & 12.4 & 7.8   & 11.1  & 16.1  & 12.2  & 16.1 & 13.0  & 188                      \\
                                                                            & CoTTA          & 15.6  & 13.6 & 17.3  & 9.8   & 19.0  & 11.0  & 10.2 & 13.5 & 12.6  & 17.4 & 7.8   & 17.3  & 16.2  & 12.9  & 16.0 & 14.0  & 409                     \\
                                                                            & EcoTTA (K=4)     & 16.1  & 13.2 & 18.3  & 8.0   & 18.3  & 9.3   & 8.6  & 10.5 & 10.1  & 12.2 & 6.8   & 11.3  & 14.5  & 11.0  & 14.8 & 12.2  & 80                       \\
                                                                            & EcoTTA (K=5)     & 15.9  & 12.6 & 17.2  & 8.2   & 18.4  & 9.3   & 8.6  & 10.6 & 10.4  & 12.4 & 6.7   & 11.7  & 14.3  & 11.3  & 14.9 & \textbf{12.1}  & 92                       \\ 
\toprule
\multirow{11}{*}{WRN28}                                                     & Source         & 72.3  & 65.7 & 72.9  & 46.9  & 54.3  & 34.8  & 42.0 & 25.1 & 41.3  & 26.0 & 9.3   & 46.7  & 26.6  & 58.5  & 30.3 & 43.5  & 37                       \\
                                                                            & tBN            & 28.6  & 26.8 & 37.0  & 13.2  & 35.4  & 14.4  & 12.6 & 18.0 & 18.2  & 16.0 & 8.6   & 13.3  & 24.0  & 20.3  & 27.8 & 20.9  & 37                       \\
                                                                            & TENT online    & 25.2  & 23.8 & 33.5  & 12.8  & 32.3  & 14.1  & 11.7 & 16.4 & 17.0  & 14.4 & 8.4   & 12.2  & 22.8  & 18.0  & 24.8 & 19.2  & 646                      \\
                                                                            & TENT continual & 25.2  & 20.8 & 29.8  & 14.4  & 31.5  & 15.4  & 14.2 & 18.8 & 17.5  & 17.3 & 10.9  & 14.9  & 23.6  & 20.2  & 25.6 & 20.0  & 646                      \\
                                                                            & TTT++*         & 27.9  & 25.8 & 35.8  & 13.0  & 34.3  & 14.2  & 12.2 & 17.4 & 17.6  & 15.5 & 8.6   & 13.1  & 23.1  & 19.6  & 26.6 & 20.3  & 1405                     \\
                                                                            & SWRNSP         & 24.6  & 20.5 & 29.3  & 12.4  & 31.1  & 13.0  & 11.3 & 15.3 & 14.7  & 11.7 & 7.8   & 9.3   & 21.5  & 15.6  & 20.3 & 17.2  & 1551                    \\
                                                                            & NOTE           & 30.4  & 26.7 & 34.6  & 13.6  & 36.3  & 13.7  & 13.9 & 17.2 & 15.8  & 15.2 & 9.1   & 7.5   & 24.1  & 18.4  & 25.9 & 20.2  & 646                      \\
                                                                            & ETAT           & 23.8  & 18.8 & 27.3  & 13.9  & 29.7  & 16.0  & 13.3 & 18.0 & 16.9  & 15.7 & 10.5  & 12.2  & 22.9  & 17.1  & 23.0 & 18.6  & 646                      \\
                                                                            & CoTTA          & 24.6  & 21.6 & 26.5  & 12.1  & 28.0  & 13.0  & 10.9 & 15.3 & 14.6  & 13.6 & 8.1   & 12.2  & 20.0  & 14.9  & 19.5 & 17.0  & 1697                    \\
                                                                            & EcoTTA (K=4)     & 23.5  & 19.0 & 26.6  & 11.5  & 30.6  & 13.1  & 10.9 & 15.2 & 14.5  & 13.1 & 7.8   & 11.4  & 20.9  & 15.4  & 20.8 & 16.9  & 404                      \\
                                                                            & EcoTTA (K=5)     & 23.8  & 18.7 & 25.7  & 11.5  & 29.8  & 13.3  & 11.3 & 15.3 & 15.0  & 13.0 & 7.9   & 11.3  & 20.2  & 15.1  & 20.5 & \textbf{16.8}  & 471                      \\ 
\toprule
\multirow{10}{*}{Resnet50}                                                  & Source         & 65.6  & 60.7 & 74.4  & 28.9  & 79.9  & 46.0  & 25.7 & 35.0 & 49.4  & 54.7 & 13.0  & 83.2  & 41.2  & 46.7  & 27.7 & 48.8  & 24                       \\
                                                                            & tBN            & 18.0  & 17.2 & 29.3  & 10.7  & 27.2  & 15.5  & 8.9  & 16.7 & 14.6  & 21.0 & 9.3   & 12.7  & 20.9  & 12.4  & 14.8 & 16.6  & 24                       \\
                                                                            & TENT online    & 16.6  & 15.7 & 25.7  & 10.0  & 24.8  & 13.8  & 8.3  & 14.9 & 13.8  & 17.6 & 8.7   & 10.0  & 19.1  & 11.5  & 13.8 & 15.0  & 925                      \\
                                                                            & TENT continual & 16.6  & 14.4 & 22.9  & 10.4  & 22.6  & 13.4  & 10.3 & 15.8 & 14.6  & 18.0 & 10.5  & 11.7  & 18.4  & 13.1  & 15.3 & 15.2  & 925                      \\
                                                                            & TTT++          & 18.2  & 16.9 & 28.7  & 10.5  & 26.5  & 14.5  & 8.9  & 16.5 & 14.5  & 20.9 & 9.0   & 9.0   & 20.4  & 12.3  & 14.7 & 16.1  & 1877                     \\
                                                                            & SWRNSP         & 17.3  & 16.1 & 26.1  & 10.6  & 25.6  & 14.1  & 8.7  & 15.6 & 13.6  & 18.6 & 8.8   & 10.0  & 19.3  & 12.0  & 14.2 & 15.4  & 1971                    \\
                                                                            & ETAT           & 17.2  & 14.9 & 23.6  & 10.2  & 23.3  & 13.2  & 8.5  & 14.0 & 12.5  & 16.6 & 8.6   & 9.4   & 17.2  & 11.0  & 12.7 & 14.2  & 925                      \\
                                                                            & CoTTA          & 16.2  & 15.0 & 21.2  & 10.4  & 22.8  & 13.9  & 8.4  & 15.1 & 12.9  & 19.8 & 8.6   & 11.3  & 17.5  & 10.5  & 12.2 & 14.4  & 2066                    \\
                                                                            & EcoTTA (K=4)     & 16.5  & 14.5 & 24.3  & 9.7   & 23.7  & 13.3  & 8.8  & 14.7 & 12.9  & 17.0 & 9.1   & 9.4   & 17.6  & 11.4  & 13.1 & 14.4  & 296                      \\
                                                                            & EcoTTA (K=5)     & 16.6  & 14.4 & 23.6  & 9.8   & 23.4  & 12.7  & 8.6  & 14.5 & 12.6  & 16.6 & 8.7   & 9.0   & 17.0  & 11.3  & 12.6 & \textbf{14.1}  & 498                      \\
\toprule
\end{tabular}}
\footnotesize
\vspace{-0.3cm}
\caption{Comparison of error rate ($\%$) on \textbf{CIFAR-10-C} with severity level 5}
\arrayrulecolor{black}
\end{table*}}

==> table/supple_full_cifar100.tex <==
{\renewcommand{\arraystretch}{.95}
\begin{table*}
\centering
\arrayrulecolor{black}
\resizebox{.98\textwidth}{!}{
\begin{tabular}{l|l|ccccccccccccccc|c|c|} 
\toprule
\textbf{Backbone}                                                                        & \textbf{Method}         & Gaus. & Shot & Impu. & Defo. & Glas. & Moti. & Zoom & Snow & Fros. & Fog  & Brig. & Cont. & Elas. & Pixe. & Jpeg &  \textbf{Avg. err {\scriptsize $\downarrow$}} & \textbf{Mem. {\scriptsize $\downarrow$}}     \\ 
\drule
\multirow{11}{*}{\begin{tabular}[c]{@{}l@{}}WRN40 \\(Aug Mix)\end{tabular}} & Source         & 80.1  & 77.0 & 76.4  & 59.9  & 77.6  & 64.2  & 59.3 & 64.8 & 71.3  & 78.3 & 48.1  & 83.4  & 65.8  & 80.4  & 59.2 & 69.7  & 2                        \\
                                                                            & tBN            & 45.9  & 45.6 & 48.2  & 33.6  & 47.9  & 34.5  & 34.1 & 40.3 & 40.4  & 47.1 & 31.7  & 39.7  & 42.7  & 39.2  & 45.6 & 41.1  & 2                        \\
                                                                            & TENT online    & 41.2  & 40.6 & 42.2  & 30.9  & 43.4  & 31.8  & 30.6 & 35.3 & 36.2  & 40.1 & 28.5  & 35.5  & 39.1  & 33.9  & 41.7 & 36.7  & 188                      \\
                                                                            & TENT continual & 41.2  & 38.2 & 41.0  & 32.9  & 43.9  & 34.9  & 33.2 & 37.7 & 37.2  & 41.5 & 33.2  & 37.2  & 41.1  & 35.9  & 45.1 & 38.3  & 188                      \\
                                                                            & TTT++*         & 46.0  & 45.4 & 48.2  & 33.5  & 47.7  & 34.4  & 33.8 & 39.9 & 40.2  & 47.1 & 31.8  & 39.7  & 42.5  & 38.9  & 45.5 & 41.0  & 391                      \\
                                                                            & SWRNSP         & 42.4  & 40.9 & 42.7  & 30.6  & 43.9  & 31.7  & 31.3 & 36.1 & 36.2  & 41.5 & 28.7  & 34.1  & 39.2  & 33.6  & 41.3 & 36.6  & 400                     \\
                                                                            & NOTE           & 50.9  & 47.4 & 49.0  & 37.3  & 49.6  & 37.3  & 37.0 & 41.3 & 39.9  & 47.0 & 35.2  & 34.7  & 45.2  & 40.9  & 49.9 & 42.8  & 188                      \\
                                                                            & ETAT           & 41.6  & 39.9 & 41.2  & 31.7  & 44.0  & 32.4  & 31.9 & 36.2 & 36.8  & 39.7 & 29.1  & 34.4  & 39.9  & 34.2  & 42.2 & 37.1  & 188                      \\
                                                                            & CoTTA          & 43.5  & 41.7 & 43.7  & 32.2  & 43.7  & 32.8  & 32.2 & 38.5 & 37.6  & 45.9 & 29.0  & 38.1  & 39.2  & 33.8  & 39.4 & 38.1  & 409                     \\
                                                                            & EcoTTA (K=4)     & 42.7  & 39.6 & 42.4  & 31.4  & 42.9  & 31.9  & 30.8 & 35.1 & 34.8  & 40.7 & 28.1  & 35.0  & 37.5  & 32.1  & 40.5 & 36.4  & 80                       \\
                                                                            & EcoTTA (K=5)     & 41.8  & 39.0 & 41.9  & 31.2  & 42.7  & 32.5  & 31.0 & 35.0 & 35.0  & 39.9 & 28.8  & 34.5  & 37.5  & 32.8  & 40.5 & \textbf{36.3}  & 92                       \\ 
\toprule
\multirow{10}{*}{Resnet50}                                                  & Source         & 84.7  & 83.5 & 93.3  & 59.6  & 92.5  & 71.9  & 54.8 & 66.6 & 77.6  & 81.8 & 44.3  & 91.2  & 72.2  & 76.6  & 56.5 & 73.8  & 24                       \\
                                                                            & tBN            & 48.1  & 46.7 & 60.6  & 35.1  & 58.0  & 41.8  & 33.2 & 47.3 & 43.5  & 54.9 & 33.5  & 35.3  & 49.8  & 38.4  & 40.8 & 44.5  & 24                       \\
                                                                            & TENT online    & 44.1  & 42.7 & 53.9  & 32.6  & 52.0  & 37.5  & 30.5 & 43.4 & 40.2  & 45.7 & 30.4  & 31.4  & 45.1  & 35.0  & 37.6 & 40.1  & 926                     \\
                                                                            & TENT continual & 44.0  & 40.1 & 49.9  & 34.7  & 50.6  & 40.0  & 33.6 & 47.0 & 45.7  & 53.4 & 42.5  & 46.2  & 56.1  & 51.2  & 53.3 & 45.9  & 926                     \\
                                                                            & TTT++          & 48.1  & 46.5 & 60.8  & 35.1  & 57.8  & 41.6  & 32.9 & 46.8 & 43.3  & 55.0 & 33.3  & 34.0  & 50.0  & 38.1  & 40.6 & 44.2  & 1876                    \\
                                                                            & SWRNSP         & 48.3  & 46.5 & 60.5  & 35.1  & 57.9  & 41.7  & 32.9 & 47.1 & 43.5  & 54.7 & 33.5  & 35.1  & 49.9  & 38.3  & 40.7 & 44.1  & 1970                   \\
                                                                            & ETAT           & 44.8  & 41.9 & 52.6  & 33.0  & 51.1  & 37.8  & 30.3 & 43.0 & 40.1  & 45.1 & 30.1  & 31.8  & 45.2  & 35.2  & 37.4 & 39.9  & 926                     \\
                                                                            & CoTTA          & 43.6  & 42.8 & 50.4  & 34.2  & 51.6  & 39.2  & 31.4 & 43.4 & 39.6  & 47.4 & 31.3  & 32.2  & 43.4  & 35.8  & 36.7 & 40.2  & 2064                   \\
                                                                            & EcoTTA (K=4)     & 46.4  & 40.7 & 50.2  & 31.1  & 48.7  & 35.2  & 29.4 & 40.8 & 39.6  & 45.3 & 30.8  & 35.8  & 44.1  & 36.4  & 38.7 & 39.5  & 296                     \\
                                                                            & EcoTTA (K=5)     & 46.4  & 41.0 & 49.1  & 31.3  & 48.9  & 35.6  & 29.6 & 41.2 & 38.5  & 44.4 & 30.7  & 35.1  & 43.5  & 36.2  & 38.8 & \textbf{39.3}  & 498                     \\
\toprule
\end{tabular}}
\footnotesize
\vspace{-0.3cm}
\caption{Comparison of error rate ($\%$) on \textbf{CIFAR-100-C} with severity level 5}
\arrayrulecolor{black}
\end{table*}}
